Do Good, Stay Longer? Temporal Patterns and Predictors of Newcomer-to-Core Transitions in Conventional OSS and OSS4SG

Open Source Software (OSS) sustainability relies on newcomers transitioning to core contributors, but this pipeline is broken, with most newcomers becoming inactive after initial contributions. Open Source Software for Social Good (OSS4SG) projects, which prioritize societal impact as their primary mission, may be associated with different newcomer-to-core transition outcomes than conventional OSS projects. We compared 375 projects (190 OSS4SG, 185 OSS), analyzing 92,721 contributors and 3.5 million commits. OSS4SG projects retain contributors at 2.2X higher rates and contributors have 19.6% higher probability of achieving core status. Early broad project exploration predicts core achievement (22.2% importance); conventional OSS concentrates on one dominant pathway (61.62% of transitions) while OSS4SG provides multiple pathways. Contrary to intuition, contributors who invest time learning the project before intensifying their contributions (Late Spike pattern) achieve core status 2.4-2.9X faster (21 weeks) than those who contribute intensively from day one (Early Spike pattern, 51-60 weeks). OSS4SG supports two effective temporal patterns while only Late Spike achieves fastest time-to-core in conventional OSS. Our findings suggest that finding a project aligned with personal values and taking time to understand the codebase before major contributions are key strategies for achieving core status. Our findings show that project mission is associated with measurably different environments for newcomer-to-core transitions and provide evidence-based guidance for newcomers and maintainers.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> tables/Commit_dataset_info.tex <==
% Requires \usepackage{graphicx} (for \resizebox)
\begin{table}[t]
\centering
\caption{Commit Metrics Extracted for Analysis}
\label{tab:commit_metrics}
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{Metric} & \textbf{Description} \\
\midrule
\multirow{7}{*}{Basic Information} 
& project\_name & Repository identifier \\
& project\_type & OSS or OSS4SG classification \\
& commit\_hash & Unique commit identifier \\
& author\_name & Contributor name \\
& author\_email & Contributor email \\
& commit\_date & Timestamp of commit (ISO) \\
& commit\_message & Commit message text \\
\midrule
\multirow{2}{*}{commit Message Metrics}
& message\_length\_chars & Character count of message \\
& message\_length\_words & Word count of message \\
\midrule
\multirow{5}{*}{File Change Metrics}
& files\_modified\_count & Number of files changed \\
& total\_insertions & Lines added \\
& total\_deletions & Lines removed \\
& total\_lines\_changed & Total lines modified \\
& churn\_ratio & Deletions-to-insertions ratio \\
\midrule
\multirow{7}{*}{Temporal Metrics}
& commit\_hour & Hour of day (0--23) \\
& commit\_day\_of\_week & Day of week (0--6) \\
& commit\_day\_of\_month & Day of month (1--31) \\
& commit\_day\_of\_year & Day of year (1--366) \\
& commit\_month & Month (1--12) \\
& commit\_year & Year \\
& commit\_is\_weekend & Boolean weekend indicator \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/Milestones_result_for_oss_and_oss4sg.tex <==

\begin{table}[h]
\centering
\caption{Milestone achievement rates by ecosystem}
\label{tab:milestone_coverage}
\begin{tabular}{lcc}
\toprule
\textbf{Milestone} & \textbf{OSS (\%)} & \textbf{OSS4SG (\%)} \\
\midrule
First Merged Pull Request (FMPR) & 52.9 & 58.9 \\
Sustained Participation 12w (SP12W) & 19.1 & 46.7 \\
Failure Recovery Resilience (FRR) & 25.1 & 40.7 \\
Return After Extended Absence (RAEA) & 12.8 & 15.5 \\
High Acceptance Trajectory (HART) & 47.4 & 54.6 \\
Direct Commit Access Proxy (DCA) & 3.2 & 13.4 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/RQ1_effort_and_time_threshholder.tex <==
\begin{table}[t]
\centering
\caption{Sensitivity: excluding early-core cases (exclude cores $\leq$ X weeks after first commit).}
\label{tab:step6_thresholds}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Threshold} & \textbf{Excluded} & \textbf{Core (\%)} & \textbf{OSS med. weeks} & \textbf{OSS med. commits} & \textbf{OSS4SG med. weeks} & \textbf{OSS4SG med. commits} & \textbf{Ratio} \\
\midrule
None        & 0       & 22.5 & 0   & 1 & 22  & 41  & 41.0x \\
$\leq$0w    & 13{,}297 & 10.6 & 52  & 2 & 32  & 55  & 27.5x \\
$\leq$1w    & 13{,}894 & 10.0 & 55  & 2 & 35  & 60  & 30.0x \\
$\leq$2w    & 14{,}275 & 9.5  & 58  & 2 & 38  & 64  & 32.0x \\
$\leq$4w    & 14{,}797 & 9.0  & 67  & 3 & 41  & 70  & 23.3x \\
$\leq$8w    & 15{,}341 & 8.4  & 76  & 2 & 47  & 76  & 38.0x \\
$\leq$12w   & 15{,}759 & 7.9  & 82  & 2 & 54  & 81  & 40.5x \\
$\leq$26w   & 16{,}827 & 6.8  & 103 & 2 & 74  & 88  & 44.0x \\
$\leq$52w   & 18{,}231 & 5.1  & 132 & 2 & 107 & 104 & 52.2x \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/RQ2_milestones_table_definitions_and_how_.tex <==
\begin{table}[H]
\centering
\begin{tabular}{|l|p{3cm}|p{4cm}|p{3cm}|}
\hline
\textbf{Milestone} & \textbf{What It Measures} & \textbf{How We Measure It} & \textbf{Why It Matters} \\
\hline
First Accepted & First successful contribution & First week with accepted commit/PR & Foundation for further engagement \\
\hline
first Sustained Participation & Consistent engagement over time & Maintained activity for 12+ consecutive weeks & Shows long-term commitment \mohamed{there was a paper that i got the number 3 motnh from}\\
\hline
Returning Contributor & Coming back after initial activity & Return to activity after initial period & Indicates sustained interest \\
\hline
Cross-Boundary & Contributing to different areas & Activity across multiple project components & Demonstrates project understanding \\
\hline
Failure Recovery & Bouncing back from setbacks & Successful contribution after rejection & Shows resilience and learning \\
\hline
\end{tabular}
\caption{5 Working Milestones: Definition, Measurement, and Significance}
\end{table}

==> tables/RQ2_milestpone_results.tex <==
\begin{table}[H]
\centering
\small
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Milestone} & \textbf{OSS Rate \%} & \textbf{OSS4SG Rate \%} & \textbf{OSS Median (wks)} & \textbf{OSS4SG Median (wks)} \\
\hline
First Accepted & 52.9 & 58.9 & 1 & 1 \\
\mohamed{}Sustained Participation & 43.7 & 94.5 & 2 & 1 \\
Returning Contributor & 33.2 & 51.6 & 13 & 13 \\
Cross-Boundary & 46.5 & 90.0 & 1 & 1 \\
Failure Recovery & 22.2 & 39.1 & 3 & 6 \\
\hline
\end{tabular}
\caption{Milestone achievement rates and median time-to-milestone by project type. Total contributors: OSS = 4,685; OSS4SG = 1,845 (6,530 total).}
\end{table}

==> tables/RQ2_treatment_metrics_definition.tex <==

\begin{table}[H]
\centering
\small
\begin{tabular}{|p{0.3\linewidth}|p{0.65\linewidth}|}
\hline
\textbf{PARTICIPATION METRICS (17)} & total\_items, items\_with\_responses, response\_rate, total\_responses, first\_response\_count, maintainer\_response\_rate, peer\_response\_rate, external\_response\_rate, re\_engagement\_cycles, total\_prs, merge\_rate, close\_rate, approval\_rate, rejection\_rate, author\_attribution\_rate, total\_issues, re\_engagement\_rate \\
\hline
\textbf{RESPONSE TIMING (20)} & first\_response\_mean\_hours, first\_response\_median\_hours, first\_response\_std\_hours, first\_response\_min\_hours, first\_response\_max\_hours, first\_response\_25th\_percentile, first\_response\_75th\_percentile, avg\_response\_mean\_hours, avg\_response\_median\_hours, avg\_response\_std\_hours, weekend\_response\_rate, off\_hours\_response\_rate, business\_hours\_response\_rate, within\_hour\_response\_rate, same\_day\_response\_rate \\
\hline
\end{tabular}
\caption{Participation Metrics and Response Timing Metrics}
\end{table}

\begin{table}[H]
\centering
\small
\begin{tabular}{|p{0.3\linewidth}|p{0.65\linewidth}|}
\hline
\textbf{RESPONSE TIMING (cont.)} & approval\_speed\_mean\_hours, approval\_speed\_median\_hours, approval\_speed\_std\_hours, approval\_speed\_min\_hours, approval\_speed\_max\_hours \\
\hline
\textbf{ENGAGEMENT BREADTH (9)} & unique\_responders, unique\_pr\_responders, repeat\_engagers, avg\_prs\_per\_responder, max\_prs\_per\_responder, response\_diversity\_index, response\_concentration\_ratio, unique\_responder\_roles, role\_diversity\_index \\
\hline
\textbf{INTERACTION PATTERNS (19)} & conversation\_length\_mean, conversation\_length\_median, conversation\_length\_std, conversation\_length\_max, conversation\_length\_min, back\_forth\_turns\_mean, back\_forth\_turns\_median, back\_forth\_turns\_std, back\_forth\_turns\_max, word\_count\_mean, word\_count\_median, word\_count\_std, word\_count\_max, sentence\_count\_mean, sentence\_count\_median, total\_messages, question\_rate, link\_sharing\_rate, avg\_words\_per\_message \\
\hline
\end{tabular}
\caption{Engagement Breadth and Interaction Patterns Metrics}
\end{table}

\begin{table}[H]
\centering
\small
\begin{tabular}{|p{0.3\linewidth}|p{0.65\linewidth}|}
\hline
\textbf{RECOGNITION SIGNALS (14)} & code\_sharing\_rate, mention\_rate, code\_snippets\_total, external\_links\_total, internal\_links\_total, thanks\_rate, praise\_rate, emoji\_usage\_rate, positive\_sentiment\_rate, positive\_emoji\_count, negative\_emoji\_count, emoji\_sentiment\_ratio, review\_requests\_received, at\_mentions \\
\hline
\textbf{TRUST INDICATORS (12)} & issue\_assignments, label\_additions, milestone\_assignments, project\_assignments, collaborative\_edits, delegated\_tasks, trusted\_with\_sensitive, pr\_with\_labels\_rate, pr\_with\_milestones\_rate, issue\_assignment\_rate, administrative\_actions, trust\_score \\
\hline
\end{tabular}
\caption{Recognition Signals and Trust Indicators Metrics}
\end{table}

==> tables/milestones_and_there_definitions.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{p{0.28\linewidth}p{0.66\linewidth}}
\hline
\textbf{Milestone} & \textbf{Meaning} \\
\hline
Newcomer & First visible participation in the project (e.g., first PR/issue/comment/commit). \\
First accepted code change & First PR merged or patch accepted, establishing initial technical trust. \\
Regular contributor & Sustained, repeated accepted contributions over time (commits/PRs). \\
Reviewer & First review submitted on others' PRs; participates in review discussions. \\
Issue participant & Opens and engages on bug reports or feature requests. \\
Issue triager & Confirms/labels/diagnoses issues; helps prioritize and clarify reports. \\
Community assistance & Helps users/newcomers (answers questions, docs improvements, guidance). \\
Relationship with project/org & Contributes across related repositories in the same org and/or shows relevant affiliation. \\
Project comprehension & Demonstrates broad understanding (e.g., coherent feature proposals, stable merge ratio, appropriate scope). \\
Nomination (candidate committer) & Formally nominated (self/sponsor/community) per governance policy. \\
Core / Committer & Granted commit rights (listed as committer/collaborator; can land changes). \\
\hline
\end{tabular}
\caption{Milestones from newcomer to core/committer and their meanings.}
\label{tab:milestones}
\end{table}


==> tables/ml_models_and_the_results.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Model} & \textbf{ROC AUC} & \textbf{PR AUC} & \textbf{Performance} \\
\hline
Random Forest & 0.746 ± 0.008 & 0.657 ± 0.008 & Best \\
Gradient Boosting & 0.746 ± 0.009 & 0.656 ± 0.009 & Second Best \\
Logistic Regression & 0.689 ± 0.009 & 0.622 ± 0.011 & Baseline \\
\hline
\end{tabular}
\caption{Model Performance on Core Contributor Prediction}
\label{tab:ml_results}
\end{table}
